Adapting Vision Foundation Models for Real-time Ultrasound Image Segmentation

We propose a novel approach that adapts hierarchical vision foundation models for real-time ultrasound image segmentation. Existing ultrasound segmentation methods often struggle with adaptability to new tasks, relying on costly manual annotations, while real-time approaches generally fail to match state-of-the-art performance. To overcome these limitations, we introduce an adaptive framework that leverages the vision foundation model Hiera to extract multi-scale features, interleaved with DINOv2 representations to enhance visual expressiveness. These enriched features are then decoded to produce precise and robust segmentation. We conduct extensive evaluations on six public datasets and one in-house dataset, covering both cardiac and thyroid ultrasound segmentation. Experiments show that our approach outperforms state-of-the-art methods across multiple datasets and excels with limited supervision, surpassing nnUNet by over 20\% on average in the 1\% and 10\% data settings. Our method achieves $\sim$77 FPS inference speed with TensorRT on a single GPU, enabling real-time clinical applications.

==> meeting.tex <==
% 1. Introduce multiple vision encoders (DINOv2, SAM2, CLIP)
% 2. Distilling multiple vision encoders to one
% 3. Test on small datasets. and the challenging inhouse thyroid datasets

==> sections/archived/results.tex <==
\section{Results}

\subsection{Cardiac dataset}
\input{tables/archived/cardiac_dataset_2d}
\input{tables/archived/cardiac_dataset_2dx}
\input{tables/archived/cardiac_dataset_fuse}

\subsection{Thyroid dataset}
\input{tables/archived/thyroid_dataset}
\input{tables/archived/thyroid_dataset2}
\input{tables/archived/uih_dataset}

% \subsection{Effectiveness on DINOv2 encoder}
% \input{tables/cardiac_dataset}

% % \subsection{Ablation on DINOv2 architectures in few-shot setting}
% % \input{tables/DINOv2_few_shot_cardiacUS}

% \subsection{Effectiveness on domain adaptation}
% \input{tables/cardiac_dataset_da}

% \subsection{Ablations on nnUNet}
% \input{tables/nnUNet_ablation}
% \input{tables/nnUNetDINO_bot_ablation}

% \subsection{Effectiveness on Thyroid datasets}
% \input{tables/thyroid_inference_speed}
% \input{tables/thyroid_dataset_description}
% \input{tables/thyroid_dataset}
% \input{tables/thyroid_dataset2}

% \subsection{Ablations on AdapterX}
% \input{tables/adapterx_ablation}
% \input{tables/cardiac_ACDC}
% \input{tables/sam2_adapter_ablation}

==> tables/ablation.tex <==
\begin{table}[tb]
    \centering
    \caption{Ablation study evaluating key components of our method: (1) Hierarchical decoder (H-Dec.), (2) Hiera adapter (H-Adp.), (3) DINOv2 feature integration, and (4) Feature interleaving. Units: DSC (\%), HD (px). Best results are in bold.}
    \begin{adjustbox}{scale=1}
    \begin{tabular}{cccc|cc}
    \toprule
    % & & & & \multicolumn{2}{c|}{CAMUS} \\
    
    % \cmidrule(lr){5-6} \cmidrule(lr){7-8}
    % \multicolumn{3}{c}{Components} &  \\
    H-Dec. & H-Adp. & DINOv2 & Interleave & DSC $\uparrow$ & HD $\downarrow$ \\
    \midrule%\midrule
    \xmark & \xmark & \xmark & \xmark & 78.23 & 30.98\\
    \cmark & \xmark & \xmark & \xmark & 90.85 & 9.42\\
    \cmark & \cmark & \xmark & \xmark & 91.89 & 6.84\\
    \cmark & \cmark & \cmark & \xmark & 91.90 & 6.78\\
    \cmark & \cmark & \cmark & \cmark & \textbf{92.01} & \textbf{6.75}\\
    \bottomrule%\bottomrule
    \end{tabular}
    \end{adjustbox}
    \label{tab:ablation}
\end{table}

==> tables/archived/adapterx_ablation.tex <==
\begin{table}[htbp]
    \centering
    \begin{adjustbox}{scale=0.73}
    \begin{tabular}{lccccc|cc}
    \toprule
    & & & & \multicolumn{2}{c|}{CAMUS} & \multicolumn{2}{c}{Site G}\\
    
    \cmidrule(lr){5-6} \cmidrule(lr){7-8}
    
    & aug & $d_{\text{adp}}$ & $N_f$ & DSC $\uparrow$ & HD $\downarrow$ & DSC $\uparrow$ & HD $\downarrow$ \\
    \midrule\midrule
    DINOv2-AIM & \xmark & 192 & 8 & 86.07 & 21.83 &  \\
    DINOv2-AIM & \xmark & 96 & 8 & 86.01 & 25.08 \\
    DINOv2-AIM & \xmark & 48 & 8 & 86.16 & 22.62 &  \\
    DINOv2-AIM & \xmark & 24 & 8 & 85.98 & 24.20 &  \\\midrule
    DINOv2-AIM & \xmark & 192 & 16 & 86.62  & 24.68 & \\
    DINOv2-AIM & \xmark & 48 & 16 & 86.34 & 26.59 & \\ \midrule
    DINOv2-AIM & \cmark & 192 & 16 & \textbf{91.38} & \textbf{9.24} \\
    \bottomrule\bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Quantitative evaluation on cardiac ultrasound datasets was performed using Dice Score (DSC) and Hausdorff Distance (HD), averaged across left and right ventricles. Units: DSC (\%), HD (px).}
    \label{tab:dinov2_aim_ablation}
\end{table}

==> tables/archived/cardiac_ACDC.tex <==
\begin{table}[htbp]
    \centering
    \begin{adjustbox}{scale=0.73}
    \begin{tabular}{lcccccccccc}
    \toprule
    & & &  \multicolumn{8}{c}{ACDC} \\
    
    \cmidrule(lr){4-11} 
    
    & & & \multicolumn{2}{c}{LV} & \multicolumn{2}{c}{Myo} & \multicolumn{2}{c}{RV}  & \multicolumn{2}{c}{Avg} \\

    \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} 

    & Loss & RandAug & DSC $\uparrow$ & HD $\downarrow$ & DSC $\uparrow$ & HD $\downarrow$ & DSC $\uparrow$ & HD $\downarrow$ & DSC $\uparrow$ & HD $\downarrow$ \\\midrule\midrule
    
    DINOv2LoRA & Dice  & torchio & 91.67 & 2.61 & 84.60 & 2.96 & \textbf{85.51} & 5.25 & 87.26 & 3.61\\
    DINOv2LoRA & Dice + CE & torchio & 90.77 & \textbf{2.56} & 84.22 & \textbf{2.95} & 84.91 & 5.08 & 86.63 & \textbf{3.53}\\
    DINOv2LoRA & Dice + CE & monai & \textbf{91.90} & 2.60 & \textbf{85.15} & 3.00 & 85.14 & \textbf{5.01} & \textbf{87.40} & 3.54\\
    % DINOv2-reg + UNetDec \\
        \bottomrule\bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Quantitative evaluation on cardiac ultrasound datasets was performed using Dice Score (DSC) and Hausdorff Distance (HD), averaged across left and right ventricles. Units: DSC (\%), HD (px).}
    \label{tab:us_seg_prelim}
\end{table}

==> tables/archived/cardiac_dataset.tex <==
\begin{table}[htbp]
    \centering
    \begin{adjustbox}{scale=0.73}
    \begin{tabular}{lcccccc|cccccc}
    \toprule
    &  \multicolumn{6}{c|}{CAMUS} & \multicolumn{6}{c}{Site G}\\
    
    \cmidrule(lr){2-7} \cmidrule(lr){8-13} 
    
    & \multicolumn{2}{c}{1\%} & \multicolumn{2}{c}{10\%} & \multicolumn{2}{c|}{100\%}  & \multicolumn{2}{c}{1\%} & \multicolumn{2}{c}{10\%} & \multicolumn{2}{c}{100\%}\\

    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13} 

    & DSC $\uparrow$ & HD $\downarrow$ & DSC $\uparrow$ & HD $\downarrow$ & DSC $\uparrow$ & HD $\downarrow$ & DSC $\uparrow$ & HD $\downarrow$ & DSC $\uparrow$ & HD $\downarrow$ & DSC $\uparrow$ & HD $\downarrow$\\\midrule\midrule
    
    Vanilla UNet &  59.49 & 51.51 & 80.14 & 26.36 & 87.70 & 15.05 & 34.65 & 41.04 & 72.83 & 26.24 & 81.69 & 20.78\\
    DINOv2 + ConvDec & 69.54 & 31.53 & 80.41 & 23.09 & 85.98 & 22.04 & 56.97 & 23.69 & 69.65 & 18.04 & 76.76 & 16.21 \\
    DINOv2-reg + ConvDec & 69.38 & 31.74 & 79.37 & 25.10 & 85.65 & 22.49 & 57.85 & 21.63 & 67.71 & 17.41 & 78.33 & 17.18\\
    \midrule
    FeatUp + ConvDec & 66.90 & \textbf{29.74} & 76.95 & 26.27 & 85.94 & 19.13 & 51.02 & 39.48 & 62.61 & 19.64 & 76.06 & 33.69 \\
    % \midrule
    % UNetDINOv2 \\\midrule
    UNetFeatUp  & 62.65 & 123.92 & 84.00 & 59.93 & 90.46 & 12.50 & 23.97 & 160.30 & \textbf{76.50} & 53.78 & \textbf{85.30} & 23.80 \\
    \midrule
    DINOv2LoRA + ConvDec & \textbf{72.55} & 30.87 & \textbf{85.67} & 12.80 & 90.54 & 8.17 & \textbf{61.37} & \textbf{21.42} & 72.76 & \textbf{14.86} & 84.43 & \textbf{9.05}\\
    DINOv2AIM + ConvDec & N/A & N/A & N/A & N/A & 91.38 & 9.24\\
    
    \midrule\midrule
    SAM2 + ConvDec & N/A  & N/A & N/A & N/A & 77.93 & 31.79 \\
    SAM2 + MSConvDec & \textbf{78.70} & \textbf{22.63} & \textbf{87.89} & 13.91 & 90.85 & 9.42 \\
    SAM2Adp + ConvDec & N/A  & N/A & N/A & N/A & 92.02 & \textbf{6.62} \\
    SAM2Adp + MSConvDec & N/A  & N/A & N/A & N/A & 91.89 & 6.84 \\
    \midrule\midrule
    SAM-DINO-Concat + MSConvDec & N/A  & N/A & N/A & N/A & 91.27 & 8.22  \\
    SAM-DINO-TwoWay + MSConvDec \\
    \midrule\midrule
    SAM2-AdapterX + ConvTDec & N/A  & N/A & N/A & N/A & 90.68 & 9.62 \\
    SAM2-SAdp + ConvTDec & N/A  & N/A & N/A & N/A & \textbf{92.20} & 7.79\\
    \midrule\midrule
    nnUNet (best fold) & N/A & N/A & N/A & N/A & 91.84 & 14.42 & N/A & N/A & N/A & N/A & \textbf{90.74} & 21.30\\
    nnUNet (all folds) & N/A & N/A & N/A & N/A & 91.96 & 14.06 & N/A & N/A & N/A & N/A & 90.62 & \textbf{18.97} \\
    nnUNetDINOBot-5 (fold 0) & N/A & N/A & N/A & N/A & 90.80 & 17.68\\
    nnUNetDINOBot-8 (fold 0) & N/A & N/A & N/A & N/A & 91.40 & 15.19\\
    nnUNetDINOBot-8 (all folds) & N/A & N/A & N/A & N/A & 91.75 & 14.53\\
    nnUNetFeatUp (all folds)  & N/A & N/A & N/A & N/A & 91.77 & 14.58 \\
    % DINOv2-reg + UNetDec \\
        \bottomrule\bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Quantitative evaluation on cardiac ultrasound datasets was performed using Dice Score (DSC) and Hausdorff Distance (HD), averaged across left and right ventricles. Units: DSC (\%), HD (px).}
    \label{tab:us_seg_prelim}
\end{table}

==> tables/archived/cardiac_dataset_2d.tex <==
\begin{table}[htbp]
    \centering
    \begin{adjustbox}{scale=0.73}
    \begin{tabular}{lcccccc|cccccc}
    \toprule
    &  \multicolumn{6}{c|}{CAMUS} & \multicolumn{6}{c}{Site G}\\
    
    \cmidrule(lr){2-7} \cmidrule(lr){8-13} 
    
    & \multicolumn{2}{c}{1\%} & \multicolumn{2}{c}{10\%} & \multicolumn{2}{c|}{100\%}  & \multicolumn{2}{c}{1\%} & \multicolumn{2}{c}{10\%} & \multicolumn{2}{c}{100\%}\\

    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13} 

    & DSC $\uparrow$ & HD $\downarrow$ & DSC $\uparrow$ & HD $\downarrow$ & DSC $\uparrow$ & HD $\downarrow$ & DSC $\uparrow$ & HD $\downarrow$ & DSC $\uparrow$ & HD $\downarrow$ & DSC $\uparrow$ & HD $\downarrow$\\\midrule\midrule
    
    Vanilla UNet &  59.49 & 51.51 & 80.14 & 26.36 & 87.70 & 15.05 & 34.65 & 41.04 & 72.83 & 26.24 & 81.69 & 20.78\\
    DINOv2 + ConvDec & 69.54 & 31.53 & 80.41 & 23.09 & 85.98 & 22.04 & 56.97 & 23.69 & 69.65 & 18.04 & 76.76 & 16.21 \\
    DINOv2-reg + ConvDec & 69.38 & 31.74 & 79.37 & 25.10 & 85.65 & 22.49 & 57.85 & 21.63 & 67.71 & 17.41 & 78.33 & 17.18\\
    \midrule
    FeatUp + ConvDec & 66.90 & \textbf{29.74} & 76.95 & 26.27 & 85.94 & 19.13 & 51.02 & 39.48 & 62.61 & 19.64 & 76.06 & 33.69 \\
    % \midrule
    % UNetDINOv2 \\\midrule
    UNetFeatUp  & 62.65 & 123.92 & 84.00 & 59.93 & 90.46 & 12.50 & 23.97 & 160.30 & \textbf{76.50} & 53.78 & \textbf{85.30} & 23.80 \\
    \midrule
    nnUNetFeatUp  & N/A & N/A & N/A & N/A & 91.78 & 6.32 \\
    nnUNet & N/A & N/A & N/A & N/A & \textbf{91.96} & \textbf{6.14}\\
    \midrule
    DINOv2LoRA + ConvDec & \textbf{72.55} & 30.87 & \textbf{85.67} & \textbf{12.80} & 90.54 & \textbf{8.17} & \textbf{61.37} & \textbf{21.42} & 72.76 & \textbf{14.86} & 84.43 & \textbf{9.05}\\
    
    \midrule\midrule
    SAM2 + MSConvDec & \textbf{78.70} & \textbf{22.63} & \textbf{87.89} & 13.91 & \textbf{90.85} & 9.42 \\
    % DINOv2-reg + UNetDec \\
    \bottomrule\bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Quantitative evaluation on cardiac ultrasound datasets was performed using Dice Score (DSC) and Hausdorff Distance (HD), averaged across left and right ventricles. Units: DSC (\%), HD (px).}
    \label{tab:us_seg_prelim}
\end{table}

==> tables/archived/cardiac_dataset_2dx.tex <==
\begin{table}[htbp]
    \centering
    \begin{adjustbox}{scale=0.73}
    \begin{tabular}{lcc}
    \toprule
    & \multicolumn{2}{c}{CAMUS} \\
    
    \cmidrule(lr){2-3}
    
    & DSC $\uparrow$ & HD $\downarrow$  \\
    \midrule\midrule
    vanilla UNet & 87.70 & 15.05\\
    nnUNet & 91.96 & \textbf{6.14}\\
    \midrule
    DINOv2LoRA + ConvDec & 90.54 & 8.17\\
    DINOv2AIM + ConvTDec & 91.38 & 9.24 \\
    \midrule
    SAM2Adp + ConvDec  & 92.02 & 6.62   \\
    SAM2Adp + MSConvDec & 91.89 & 6.84 \\
    SAM2AdpX + ConvTDec & 92.51 & 7.75  \\
    SAM2AdpX + MSConvTDec & 92.38 & 8.03 \\
    SAM2AdpX + ConvTAttn & 92.59 & 7.38\\
    SAM2AdpX + MSConvTAttn & \textbf{92.64} & 7.75\\
    \bottomrule\bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Quantitative evaluation on cardiac ultrasound datasets was performed using Dice Score (DSC) and Hausdorff Distance (HD), averaged across left and right ventricles. Units: DSC (\%), HD (px).}
    \label{tab:dinov2_aim_ablation}
\end{table}

==> tables/archived/cardiac_dataset_da.tex <==
\begin{table}[htbp]
    \centering
    \begin{adjustbox}{scale=0.73}
    \begin{tabular}{lcccccc|cccccc}
    \toprule
    &  \multicolumn{6}{c|}{CAMUS$\rightarrow$ Site G} & \multicolumn{6}{c}{Site G $\rightarrow$ CAMUS}\\
    
    \cmidrule(lr){2-7} \cmidrule(lr){8-13} 
    
    & \multicolumn{2}{c}{1\%} & \multicolumn{2}{c}{10\%} & \multicolumn{2}{c|}{100\%}  & \multicolumn{2}{c}{1\%} & \multicolumn{2}{c}{10\%} & \multicolumn{2}{c}{100\%}\\

    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13} 

    & DSC $\uparrow$ & HD $\downarrow$ & DSC $\uparrow$ & HD $\downarrow$ & DSC $\uparrow$ & HD $\downarrow$ & DSC $\uparrow$ & HD $\downarrow$ & DSC $\uparrow$ & HD $\downarrow$ & DSC $\uparrow$ & HD $\downarrow$\\\midrule\midrule
    
    Vanilla UNet & 20.58 & 52.57 & 3.58 & 77.23 & 3.79 & 62.03 &  - & - & 9.44 & 98.74 & 11.78 & 85.67 \\
    DINOv2 + ConvDec & 22.23 & 97.08  & 16.60 & 78.01 & 9.91 & 125.39 & - & - & 0.40 & 81.63 & 4.76 & 88.39\\
    DINOv2-reg + ConvDec & 15.15 & 76.18  & 11.90 & 84.84 & 8.22 & 118.99 & - & - & 6.20 & 82.33 & 18.39 & 92.73 \\\midrule
    FeatUp + ConvDec  & 25.48 & 91.75 & 20.44 & 94.35 & 9.07 & 134.37 & - & - & 1.36 & 79.14 & 2.02 & 155.05\\
    UNetFeatUp & 18.77 & 128.46 & 16.38 & 117.31 & 12.30 & 68.46 & 12.20 & 147.53 & 2.75 & 108.87 & 10.38 & 74.29\\
    % DINOv2-reg + UNetDec \\
        \bottomrule\bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Quantitative evaluation on cardiac ultrasound datasets was performed using Dice Score (DSC) and Hausdorff Distance (HD), averaged across left and right ventricles. Units: DSC (\%), HD (px).}
    \label{tab:us_seg_prelim}
\end{table}

==> tables/archived/cardiac_dataset_fuse.tex <==
\begin{table}[htbp]
    \centering
    \begin{adjustbox}{scale=0.73}
    \begin{tabular}{lcc}
    \toprule
    & \multicolumn{2}{c}{CAMUS} \\
    
    \cmidrule(lr){2-3}
    
    & DSC $\uparrow$ & HD $\downarrow$  \\
    \midrule\midrule
    DINOv2LoRA + ConvDec & 90.54 & 8.17\\
    SAM2 + MSConvDec & 90.85 & 9.42\\
    SAM2DINO - Concat + MSConv & 91.27 & 8.22\\
    SAM2AdpDINO - Concat + MSConv & 91.90 & 6.78\\
    SAM2AdpDINO - Interleave + MSConv & \textbf{92.01} & \textbf{6.75}\\
    SAM2AdpDINOCLIP - Concat + MSConv & 91.85 & 6.70\\
    SAM2AdpDINOCLIP - Interleave + MSConv & 91.79 & 7.04\\
    SAM2AdpDINOSigLIP - Concat + MSConv & 91.09 & 7.25\\
    SAM2AdpDINOSigLIP - Interleave + MSConv & 91.68 & 6.99\\
    \bottomrule\bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Quantitative evaluation on cardiac ultrasound datasets was performed using Dice Score (DSC) and Hausdorff Distance (HD), averaged across left and right ventricles. Units: DSC (\%), HD (px).}
    \label{tab:dinov2_aim_ablation}
\end{table}

\begin{align}
    F_{fuse} = (\alpha\|F_{\text{DINOv2}}\|_2, (1-\alpha)\|F_{\text{SAM2}}\|_2)
\end{align}

==> tables/archived/nnUNetDINO_bot_ablation.tex <==
\begin{table}[htbp]
    \centering
    \begin{adjustbox}{scale=0.73}
    \begin{tabular}{lcc|cc}
    \toprule
    &  \multicolumn{2}{c|}{nnUNetDINO} & \multicolumn{2}{c}{nnUNetFeatUp}\\
    
    \cmidrule(lr){2-3} \cmidrule(lr){4-5}
    
    & DSC $\uparrow$ & HD $\downarrow$ & DSC $\uparrow$ & HD $\downarrow$ \\
    \midrule\midrule
    fold 0 & 91.40 & 15.19 & 91.36 & 15.47\\
    fold 1 & 91.48 & 15.18 & 91.53 & 15.11  \\
    fold 2 & 91.45 & 15.09 & 91.46 & 15.28 \\
    fold 3 & 91.42 & 15.28 & 91.45 & 15.34 \\
    fold 4 & 91.42 & 15.10 & 91.44 & 15.33 \\
    all folds & \textbf{91.75} & \textbf{14.53} & \textbf{91.77} & \textbf{14.58} \\
    all folds-pp & \textbf{91.75} & \textbf{14.53} & \textbf{91.77} & \textbf{14.58}\\
    \bottomrule\bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Quantitative evaluation on cardiac ultrasound datasets was performed using Dice Score (DSC) and Hausdorff Distance (HD), averaged across left and right ventricles. Units: DSC (\%), HD (px).}
    \label{tab:nnUNet_ablation}
\end{table}

==> tables/archived/nnUNet_ablation.tex <==
\begin{table}[htbp]
    \centering
    \begin{adjustbox}{scale=0.73}
    \begin{tabular}{lcc|cc}
    \toprule
    &  \multicolumn{2}{c|}{CAMUS} & \multicolumn{2}{c}{Site G}\\
    
    \cmidrule(lr){2-3} \cmidrule(lr){4-5}
    
    & DSC $\uparrow$ & HD $\downarrow$ & DSC $\uparrow$ & HD $\downarrow$ \\
    \midrule\midrule
    fold 0 & 91.69 & 14.57 & 90.38 & 21.70 \\
    fold 1 & 91.84 & 14.42 &  86.90 & 26.59 \\
    fold 2 & 91.77 & 14.52 & \textbf{90.74} & 21.30 \\
    fold 3 & 91.76 & 14.55 & 89.61 & 21.37 \\
    fold 4 & 91.72 & 14.43 & 90.55 & 23.42\\
    all folds & \textbf{91.96} & \textbf{14.06} & 90.62 & \textbf{18.97}\\
    all folds-pp & \textbf{91.96} & \textbf{14.06} & 90.62 & \textbf{18.97}\\
    \bottomrule\bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Quantitative evaluation on cardiac ultrasound datasets was performed using Dice Score (DSC) and Hausdorff Distance (HD), averaged across left and right ventricles. Units: DSC (\%), HD (px).}
    \label{tab:nnUNet_ablation}
\end{table}

==> tables/archived/sam2_adapter_ablation.tex <==
\begin{table}[htbp]
    \centering
    \begin{adjustbox}{scale=0.73}
    \begin{tabular}{lccc}
    \toprule
    & & \multicolumn{2}{c|}{CAMUS} \\
    
    \cmidrule(lr){3-4}
    
    & MLP ratio & DSC $\uparrow$ & HD $\downarrow$  \\
    \midrule\midrule
    SAM2Adp + MSConv & 0.25 & 90.85 & 9.42   \\
    SAM2Adp + MSConv & 0.125 & \textbf{91.00} & \textbf{8.31} \\
    SAM2Adp + MSConv & 0.0625 & 90.58 & 8.56  \\
    \bottomrule\bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Quantitative evaluation on cardiac ultrasound datasets was performed using Dice Score (DSC) and Hausdorff Distance (HD), averaged across left and right ventricles. Units: DSC (\%), HD (px).}
    \label{tab:dinov2_aim_ablation}
\end{table}

==> tables/archived/thyroid_dataset.tex <==
% \begin{table}[htbp]
%     \centering
%     \begin{adjustbox}{scale=0.65}
%     \begin{tabular}{lcccccc|cccccc}
%     \toprule
%     &  \multicolumn{6}{c|}{TN3K} & \multicolumn{6}{c}{TG3K}\\
    
%     \cmidrule(lr){2-7} \cmidrule(lr){8-13} 
    
%     & \multicolumn{2}{c}{1\%} & \multicolumn{2}{c}{10\%} & \multicolumn{2}{c|}{100\%}  & \multicolumn{2}{c}{1\%} & \multicolumn{2}{c}{10\%} & \multicolumn{2}{c}{100\%}\\

%     \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13} 

%     & DSC $\uparrow$ & HD95 $\downarrow$ & DSC $\uparrow$ & HD95 $\downarrow$ & DSC $\uparrow$ & HD95 $\downarrow$ & DSC $\uparrow$ & HD95 $\downarrow$ & DSC $\uparrow$ & HD95 $\downarrow$ & DSC $\uparrow$ & HD95 $\downarrow$\\\midrule\midrule
%     DINOv2LoRA + ConvDec (224) & 52.90 & 50.79 & 67.52 & 39.95 & 81.84 & 18.49 \\
%     DINOv2LoRA + ConvDec (448) & 57.16 & 55.07 & 74.55 & 34.17 & \textbf{83.91} & \textbf{16.44} & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00\\
%     % DINOv2-reg + UNetDec \\
%         \bottomrule\bottomrule
%     \end{tabular}
%     \end{adjustbox}
%     \caption{Quantitative evaluation on cardiac ultrasound datasets was performed using Dice Score (DSC) and Hausdorff Distance (HD), averaged across left and right ventricles. Units: DSC (\%), HD (px).}
%     \label{tab:us_seg_prelim}
% \end{table}

\begin{table}[htbp]
    \centering
    \begin{adjustbox}{scale=1}
    \begin{tabular}{lcc|cc}
    \toprule
    &  \multicolumn{2}{c|}{TN3K} & \multicolumn{2}{c}{DDTI}\\
    
    % \cmidrule(lr){2-7} \cmidrule(lr){8-13} 

    \cmidrule(lr){2-3} \cmidrule(lr){4-5}

    & DSC $\uparrow$ & HD95 $\downarrow$ & DSC $\uparrow$ & HD95 $\downarrow$ \\\midrule\midrule
    
    % DINOv2-reg + UNetDec \\
    UNet & 79.51 & 18.44 & 59.74 & 40.43 \\
    SGUNet & 79.55 & 18.16 & 62.92 & 34.62 \\
    TRFE & 81.19 & 17.96 & 69.04 & 34.60 \\
    FCN & 81.08 & 16.93 & 69.96 & 31.03\\
    SegNet & 79.91 & 17.13 & 65.19 & 37.32\\
    Deeplabv2 & 82.77 & 13.92 & 74.40 & 25.45\\
    CPFNet & 82.87 & 13.56 & 74.77 & 24.79\\
    TransUNet & 81.84 & 14.92 & 74.43 & \textbf{24.37}\\
    TRFE+ & 83.30 & \textbf{13.23} & 75.37 & 24.60\\
    DINOv2LoRA & 83.38  & 16.55 & 80.51 & 29.28 \\
    SAM2Adp+MSConv & \textbf{84.93} & 16.06 & \textbf{80.59} & 26.79 \\
    \bottomrule\bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Quantitative evaluation on cardiac ultrasound datasets was performed using Dice Score (DSC) and Hausdorff Distance (HD), averaged across left and right ventricles. Units: DSC (\%), HD (px).}
    \label{tab:us_seg_prelim}
\end{table}

==> tables/archived/thyroid_dataset2.tex <==
\begin{table}[htbp]
    \centering
    \begin{adjustbox}{scale=1}
    \begin{tabular}{lcc|cc}
    \toprule
    &  \multicolumn{2}{c|}{Stanford Thyroid} & \multicolumn{2}{c}{TG3K}\\
    
    % \cmidrule(lr){2-7} \cmidrule(lr){8-13} 

    \cmidrule(lr){2-3} \cmidrule(lr){4-5}

    & DSC $\uparrow$ & HD95 $\downarrow$ & DSC $\uparrow$ & HD95 $\downarrow$ \\\midrule\midrule
    
    % DINOv2-reg + UNetDec \\
    DINOv2LoRA & 90.29  & 8.78 & 78.43 & 17.48 \\
        SAM2Adp+MSConv & \textbf{96.78} & \textbf{2.75} & \textbf{84.50} & \textbf{13.23}\\
    \bottomrule\bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Quantitative evaluation on cardiac ultrasound datasets was performed using Dice Score (DSC) and Hausdorff Distance (HD), averaged across left and right ventricles. Units: DSC (\%), HD (px).}
    \label{tab:us_seg_prelim}
\end{table}

==> tables/archived/thyroid_dataset_description.tex <==
\begin{table}[htbp]
    \centering
    \begin{adjustbox}{scale=0.9}
    \begin{tabular}{lcccc}
    \toprule
    % &  \multicolumn{2}{c|}{Stanford Thyroid} & \multicolumn{2}{c}{TG3K}\\
    Dataset details & $N_{\text{train}}$ & $N_{\text{val}}$ & $N_{\text{test}}$ & Ultrasound device \\\midrule
    
    % \cmidrule(lr){2-7} \cmidrule(lr){8-13} 

    % \cmidrule(lr){2-3} \cmidrule(lr){4-5}

    % & DSC $\uparrow$ & HD95 $\downarrow$ & DSC $\uparrow$ & HD95 $\downarrow$ \\\midrule\midrule
    
    % DINOv2-reg + UNetDec \\
    TN3K (Gong et al., 2023) \cite{gong_thyroid_2023} & 2303 & 576 & 614 & GE Logiq E9, ARIETTA 850, RESONA 70B \\
    DDTI (Pedraza et al., 2015) \cite{pedraza_open_2015} & -  & - & 637 & TOSHIBA Nemio 30 and MX \\
    TG3K (Wunderling et al., 2017) \cite{wunderling_comparison_2017} & 3226 & 359 & - & GE Logiq E9\\
    Stanford (Yamashita et al., 2022) \cite{yamashita_toward_2022} & 10358 & 3453 & 3453 & GE Logiq E9, Siemens S2000\\
    \bottomrule\bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Details of thyroid dataset.}
    \label{tab:us_seg_prelim}
\end{table}

==> tables/archived/thyroid_inference_speed.tex <==
\begin{table}[htbp]
    \centering
    \begin{adjustbox}{scale=0.9}
    \begin{tabular}{lc}
    \toprule
    % &  \multicolumn{2}{c|}{Stanford Thyroid} & \multicolumn{2}{c}{TG3K}\\
    Dataset details & Inference speed (items/second) \\\midrule
    
    % \cmidrule(lr){2-7} \cmidrule(lr){8-13} 

    % \cmidrule(lr){2-3} \cmidrule(lr){4-5}

    % & DSC $\uparrow$ & HD95 $\downarrow$ & DSC $\uparrow$ & HD95 $\downarrow$ \\\midrule\midrule
    
    % DINOv2-reg + UNetDec \\
    TN3K (Gong et al., 2023) \cite{gong_thyroid_2023} & 16.18 \\
    DDTI (Pedraza et al., 2015) \cite{pedraza_open_2015} & 16.41  \\
    TG3K (Wunderling et al., 2017) \cite{wunderling_comparison_2017} & 16.20 \\
    Stanford (Yamashita et al., 2022) \cite{yamashita_toward_2022} & 16.69 \\
    \bottomrule\bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Details of thyroid dataset.}
    \label{tab:us_seg_prelim}
\end{table}

==> tables/archived/uih_dataset.tex <==
\begin{table}[htbp]
    \centering
    \begin{adjustbox}{scale=0.73}
    \begin{tabular}{lcccccc}
    \toprule
    & \multicolumn{2}{c}{Segmentation} &  \multicolumn{4}{c}{Image-level Detection}\\
    
    \cmidrule(lr){2-3} \cmidrule(lr){4-7}
    
    & DSC $\uparrow$ & HD $\downarrow$  & Prec. $\uparrow$ & Rec. $\uparrow$ & Spec. $\uparrow$ & F1 $\uparrow$ \\
    \midrule\midrule
    SAM2AdpDINOSigLIP - Concat + MSConv & 81.19 & 30.23 & 80.82 & 99.08 & 59.72 & 89.02\\
    SAM2AdpDINOSigLIP - Interleave + MSConv & 82.12 & 28.64 & 85.40 & 98.89 & 71.05 & 91.65\\
    \bottomrule\bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Quantitative evaluation on cardiac ultrasound datasets was performed using Dice Score (DSC) and Hausdorff Distance (HD), averaged across left and right ventricles. Units: DSC (\%), HD (px).}
    \label{tab:dinov2_aim_ablation}
\end{table}

\begin{align}
    F_{fuse} = (\alpha\|F_{\text{DINOv2}}\|_2, (1-\alpha)\|F_{\text{SAM2}}\|_2)
\end{align}

==> tables/camus.tex <==
\begin{table}[tb]
    \centering
    \caption{Comparison of left ventricle segmentation with SOTA methods on CAMUS dataset using Dice Score (DSC), Intersection over Union (IoU), 95th-percentile Hausdorff Distance (HD95), and Average Surface Distance (ASD). Units: DSC (\%), IoU (\%), HD95 (mm), ASD (mm). The best results are in bold, second best are in underlined.}
    % \renewcommand{\arraystretch}{1.2}
    \begin{adjustbox}{scale=0.8}
        \begin{tabular}{lcccc}
            % \hline
            \toprule
            % \multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{c}{\textbf{CAMUS}} \\
            % \cline{2-5}
            % \cmidrule{2-5}
            Method & DSC $\uparrow$ & IoU $\uparrow$ & HD95 $\downarrow$ & ASD $\downarrow$ \\
            % \hline
            \midrule
            % UNet & 90.13 & 82.36 & 5.77 & 2.35 \\
            SwinUNet & 88.84 & 80.33 & 6.10 & 2.60 \\
            H2Former & 91.31 & 84.30 & 5.27 & 2.05 \\
            \midrule
            MedSAM & 85.42 & 75.14 & 8.42 & 3.34 \\
            MSA & 88.03 & 78.98 & 7.53 & 2.85 \\
            SAMed & 87.45 & 78.14 & 9.17 & 3.10 \\
            SonoSAM & 89.80 & 81.79 & 6.60 & 2.45 \\
            % SAMUS & 91.11 & 83.94 & 5.08 & 2.07 \\
            % \midrule
            % \textbf{MemSAM} & \textbf{93.31}$\pm$\textbf{3.04} & \textbf{87.61}$\pm$\textbf{5.12} & \textbf{3.82}$\pm$\textbf{1.80} & \textbf{1.57}$\pm$\textbf{0.72} \\
            MemSAM & \underline{93.31} & \underline{87.61} & \textbf{3.82} & \textbf{1.57}\\ 
            Ours & \textbf{93.80} & \textbf{88.49} & \underline{4.80} & \underline{1.90}\\
            \bottomrule
    \end{tabular}
    \end{adjustbox}
    \label{tab:camus_sota}
\end{table}



==> tables/tn3k.tex <==
% \begin{table}[htbp]
%     \centering
%     \caption{Quantitative evaluation on cardiac ultrasound datasets was performed using Dice Score (DSC) and Hausdorff Distance (HD), averaged across left and right ventricles. Units: DSC (\%), HD (px).}
%     \begin{adjustbox}{scale=1}
%     \begin{tabular}{lcc|cc}
%     \toprule
%     &  \multicolumn{2}{c|}{Stanford Thyroid} & \multicolumn{2}{c}{TG3K}\\
    
%     % \cmidrule(lr){2-7} \cmidrule(lr){8-13} 

%     \cmidrule(lr){2-3} \cmidrule(lr){4-5}

%     & DSC $\uparrow$ & HD95 $\downarrow$ & DSC $\uparrow$ & HD95 $\downarrow$ \\\midrule\midrule
    
%     % DINOv2-reg + UNetDec \\
%     DINOv2LoRA & 90.29  & 8.78 & 78.43 & 17.48 \\
%         SAM2Adp+MSConv & \textbf{96.78} & \textbf{2.75} & \textbf{84.50} & \textbf{13.23}\\
%     \bottomrule\bottomrule
%     \end{tabular}
%     \end{adjustbox}
%     \label{tab:us_seg_prelim}
% \end{table}

% \begin{table}[h]
%     \centering
%     % \renewcommand{\arraystretch}{1.2}
%     \caption{Performance comparison of different segmentation methods. Best values are highlighted in \textbf{bold}.}
%     \begin{adjustbox}{scale=0.8}
%         \begin{tabular}{lcccc}
%         % \hline
%         \toprule
%         \textbf{Method} & \textbf{Accuracy (\%)} & \textbf{IOU (\%)} & \textbf{DSC (\%)} & \textbf{HD95} \\
%         % \hline
%         \midrule
%         Unet & 96.46 $\pm$ 0.11 & 65.99 $\pm$ 0.66 & 79.51 $\pm$ 1.31 & 18.44 $\pm$ 0.75 \\
%         TRFE & 96.71 $\pm$ 0.07 & 68.33 $\pm$ 0.68 & 81.91 $\pm$ 1.35 & 17.96 $\pm$ 1.24 \\
%         SegNet & 96.72 $\pm$ 0.12 & 66.54 $\pm$ 0.85 & 79.91 $\pm$ 1.69 & 17.13 $\pm$ 0.89 \\
%         DeepLabv3 & \textbf{97.19} $\pm$ 0.05 & 70.60 $\pm$ 0.49 & 82.77 $\pm$ 0.98 & 13.92 $\pm$ 0.89 \\
%         TRFE+ & 97.04 $\pm$ 0.10 & 71.38 $\pm$ 0.43 & 83.30 $\pm$ 0.26 & 13.23 $\pm$ 0.63 \\
%         TRFE+ w. SHAN & 96.73 $\pm$ 0.06 & \textbf{73.59} $\pm$ 0.16 & \textbf{84.61} $\pm$ 0.04 & \textbf{4.05} $\pm$ 0.27 \\
%         Ours \\
%         \bottomrule
%     \end{tabular}
%     \end{adjustbox}
%     \label{tab:camus}
% \end{table}

\begin{table}[tb]
    \centering
    % \renewcommand{\arraystretch}{1.2}
    \caption{Comparison with SOTA methods on the TN3K dataset using Accuracy (ACC), Intersection over Union (IoU), Dice Score (DSC), and 95th-percentile Hausdorff Distance (HD95). Units:  Accuracy (\%), DSC (\%), IoU (\%), HD95 (px). The best results are in bold, second best is underlined.}
    \begin{adjustbox}{scale=0.8}
        \begin{tabular}{lcccc}
        % \hline
        \toprule
        Method & ACC $\uparrow$ & IoU $\uparrow$ & DSC$\uparrow$ & HD95$\downarrow$  \\
        % \hline
        \midrule
        % Unet & 96.46 & 65.99 & 79.51 & 18.44 \\
        TRFE & 96.71 & 68.33 & 81.91 & 17.96 \\
        SegNet & 96.72 & 66.54 & 79.91 & 17.13 \\
        DeepLabv3 & 97.19 & 70.60 & 82.77 & 13.92 \\
        TRFE+ & 97.04 & 71.38 & 83.30 & \underline{13.23} \\
        %TRFE+ w. 
        SHAN & \underline{96.73} & \underline{73.59} & \underline{84.61} & \textbf{4.05} \\
        Ours & \textbf{97.60} & \textbf{78.13} & \textbf{86.01} & 15.42\\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \label{tab:tn3k_sota}
\end{table}


==> tables/uih.tex <==
% \begin{table}[htbp]
%     \centering
%     \caption{Quantitative evaluation on cardiac ultrasound datasets was performed using Dice Score (DSC) and Hausdorff Distance (HD), averaged across left and right ventricles. Units: DSC (\%), HD (px).}
%     \begin{adjustbox}{scale=0.73}
%     \begin{tabular}{lcccccc}
%     \toprule
%     & \multicolumn{2}{c}{Segmentation} &  \multicolumn{4}{c}{Image-level Detection}\\
    
%     \cmidrule(lr){2-3} \cmidrule(lr){4-7}
    
%     & DSC $\uparrow$ & HD $\downarrow$  & Prec. $\uparrow$ & Rec. $\uparrow$ & Spec. $\uparrow$ & F1 $\uparrow$ \\
%     \midrule\midrule
%     SAM2AdpDINOSigLIP - Concat + MSConv & 81.19 & 30.23 & 80.82 & 99.08 & 59.72 & 89.02\\
%     SAM2AdpDINOSigLIP - Interleave + MSConv & 82.12 & 28.64 & 85.40 & 98.89 & 71.05 & 91.65\\
%     \bottomrule\bottomrule
%     \end{tabular}
%     \end{adjustbox}
%     \label{tab:dinov2_aim_ablation}
% \end{table}

\begin{table}[tb]
    \centering
    \caption{Quantitative image-level evaluation on in-house ultrasound datasets. All values are reported as percentages (\%). The best results are highlighted in bold.}
    \label{tab:uih_detection}
    \begin{adjustbox}{scale=0.9}
    \begin{tabular}{lcccc}
    \toprule
    Model & Precision $\uparrow$ & Recall $\uparrow$ & Specificity $\uparrow$ & F1-Score $\uparrow$\\
    \midrule
    UNet \cite{ronneberger_u-net_2015}  & 64.75 & 93.92 & 12.41 & 96.86 \\
    nnUNet \cite{isensee_nnu-net_2021}     & 91.97 & 93.48 & 86.02 & 96.63 \\ \midrule
    MedNeXt \cite{greenspan_mednext_2023}    & 93.90 & 86.96 & 90.32 & 93.03 \\
    SwinUNETR \cite{greenspan_swinunetr-v2_2023}  & 62.09 & 95.61 & 0.00 & 97.75\\ \midrule
    % SonoSAM   & — & — & — & — \\
    SAMUS \cite{lin_beyond_2024}     & \textbf{100.00} & 13.23 & \textbf{100.00} & 23.37 \\
    MedSAM2 \cite{zhu_medical_2024}    & 96.67 & 85.61 & 94.95 & 92.25 \\
    Ours        & 87.21 & \textbf{98.41} & 75.27 & \textbf{99.20} \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
\end{table}

